How Infinitely Wide Neural Networks Can Benefit from Multi-task Learning -- an Exact Macroscopic Characterization

In practice, multi-task learning (through learning features shared among tasks) is an essential property of deep neural networks (NNs). While infinite-width limits of NNs can provide good intuition for their generalization behavior, the well-known infinite-width limits of NNs in the literature (e.g., neural tangent kernels) assume specific settings in which wide ReLU-NNs behave like shallow Gaussian Processes with a fixed kernel. Consequently, in such settings, these NNs lose their ability to benefit from multi-task learning in the infinite-width limit. In contrast, we prove that optimizing wide ReLU neural networks with at least one hidden layer using L2-regularization on the parameters promotes multi-task learning due to representation-learning - also in the limiting regime where the network width tends to infinity. We present an exact quantitative characterization of this infinite width limit in an appropriate function space that neatly describes multi-task learning.

==> Images/DeepStackedBasic.tex <==
\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-0.8,xscale=1]
%uncomment if require: \path (0,900); %set diagram left start at 0, and has height of 900

%Shape: Rectangle [id:dp008228614767346265] 
\draw   (73.05,219.55) -- (108.15,219.55) -- (108.15,318) -- (73.05,318) -- cycle ;
%Shape: Rectangle [id:dp5704329413062827] 
\draw   (138.96,72) -- (174.49,72) -- (174.49,410.09) -- (138.96,410.09) -- cycle ;
%Shape: Rectangle [id:dp4510734487688641] 
\draw   (209.5,259) -- (246.31,259) -- (246.31,305) -- (209.5,305) -- cycle ;
%Shape: Rectangle [id:dp02284685801621511] 
\draw   (280.42,72) -- (316.33,72) -- (316.33,411.09) -- (280.42,411.09) -- cycle ;
%Shape: Rectangle [id:dp93629233013766] 
\draw   (353.14,241.36) -- (389.05,241.36) -- (389.05,319.36) -- (353.14,319.36) -- cycle ;
%Straight Lines [id:da9888559282955649] 
\draw    (108.15,219.55) -- (138.96,72) ;
%Straight Lines [id:da09420527661413058] 
\draw    (108.15,318) -- (138.96,410.09) ;
%Straight Lines [id:da5672698781637233] 
\draw    (174.49,72) -- (209.5,259) ;
%Straight Lines [id:da9038073873782468] 
\draw    (246.31,259) -- (280.42,72) ;
%Straight Lines [id:da45145254545262614] 
\draw    (174.49,410.09) -- (209.5,305) ;
%Straight Lines [id:da5621136775375117] 
\draw    (246.31,305) -- (280.42,411.09) ;
%Straight Lines [id:da22909141129558508] 
\draw    (316.33,72) -- (353.14,241.36) ;
%Straight Lines [id:da7988859530231025] 
\draw    (316.33,411.09) -- (353.14,319.36) ;
%Shape: Rectangle [id:dp5232562566788923] 
\draw   (423.42,73) -- (459.33,73) -- (459.33,408.09) -- (423.42,408.09) -- cycle ;
%Shape: Rectangle [id:dp26495238359049167] 
\draw   (496.14,261) -- (532.05,261) -- (532.05,316.45) -- (496.14,316.45) -- cycle ;
%Straight Lines [id:da26171249376784833] 
\draw    (389.05,241.36) -- (423.42,73) ;
%Straight Lines [id:da5159016275981532] 
\draw    (389.05,319.36) -- (423.42,408.09) ;
%Straight Lines [id:da12901460002976672] 
\draw    (459.33,73) -- (496.14,261) ;
%Straight Lines [id:da3198438831389272] 
\draw    (459.33,408.09) -- (496.14,316.45) ;

% Text Node
\draw (140.42,239) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=center] {ReLU\\
($n_1$)};
% Text Node
\draw (281.98,241) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=center] {ReLU\\
($n_2$)};
% Text Node
\draw (209.24,273) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {$\quad\, \sigb$\\
\ \ ($d_1$)};
% Text Node
\draw (351.83,273) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {$\quad\ \sigb$\\
\ \ ($d_2$)};
% Text Node
\draw (76.07,261) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=center] {Input\\
($d_0$)
};
% Text Node
\draw (424.98,238) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=center] {ReLU\\
($n_3$)};
% Text Node
\draw (494.83,270) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=center] {\ Output\quad\\
$\link^{-1}$\\
($d_3$)};


\end{tikzpicture}

==> Images/shallowToOneStackGeneral.tex <==
\begin{figure}[htbp]
\centering
\begin{minipage}[t]{.3\linewidth}
\centering
\begin{adjustbox}{width=\linewidth, totalheight=1.5\linewidth}
\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,900); %set diagram left start at 0, and has height of 900

%Shape: Rectangle [id:dp9881686970179928] 
\draw   (90.05,586.55) -- (125.15,586.55) -- (125.15,685) -- (90.05,685) -- cycle ;
%Shape: Rectangle [id:dp021528437984906112] 
\draw   (155.96,458) -- (191.49,458) -- (191.49,800.73) -- (155.96,800.73) -- cycle ;
%Shape: Rectangle [id:dp9976069955613152] 
\draw   (226.5,611) -- (263.31,611) -- (263.31,657) -- (226.5,657) -- cycle ;
%Straight Lines [id:da7522636924221078] 
\draw    (125.15,586.55) -- (155.96,458) ;
%Straight Lines [id:da2407156240240318] 
\draw    (125.15,685) -- (155.96,800.73) ;
%Straight Lines [id:da5701929838169528] 
\draw    (191.49,458) -- (226.5,611) ;
%Straight Lines [id:da9714111484528329] 
\draw    (191.49,800.73) -- (226.5,657) ;

% Text Node
\draw (160.42,626) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {\scalebox{1}[1.1]{ReLU}\\ \scalebox{0.9}[1.1]{($n_j$)}};
% Text Node
\draw (229.24,627) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {\scalebox{0.9}[1.1]{$\link^{-1}$}\\
\scalebox{0.9}[1.1]{($d_j$)}};
% Text Node
\draw (95.07,626) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {\scalebox{1}[1.1]{Input}\\ \scalebox{0.9}[1.1]{($d_{j-1}$)} };

\end{tikzpicture}
\end{adjustbox}
\caption{Schematic representation of a shallow neural network, which corresponds to one stack in the main paper.}
\label{fig:shallow_nn}
\end{minipage}
\hfill
\begin{minipage}[t]{.3\linewidth}
\centering
\begin{adjustbox}{width=\linewidth, totalheight=1.5\linewidth}
\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,900); %set diagram left start at 0, and has height of 900

%Shape: Rectangle [id:dp9881686970179928] 
\draw   (124.05,689.55) -- (159.15,689.55) -- (159.15,788) -- (124.05,788) -- cycle ;
%Shape: Rectangle [id:dp021528437984906112] 
\draw   (189.96,489.09) -- (225.49,489.09) -- (225.49,732.64) -- (189.96,732.64) -- cycle ;
%Shape: Rectangle [id:dp9976069955613152] 
\draw   (260.5,714) -- (297.31,714) -- (297.31,760) -- (260.5,760) -- cycle ;
%Straight Lines [id:da7522636924221078] 
\draw    (159.15,689.55) -- (189.96,489.09) ;
%Straight Lines [id:da2407156240240318] 
\draw    (159.15,788) -- (189.96,732.64) ;
%Straight Lines [id:da5701929838169528] 
\draw    (225.49,489.09) -- (260.5,714) ;
%Straight Lines [id:da9714111484528329] 
\draw    (225.49,732.64) -- (260.5,760) ;
%Curve Lines [id:da7838414414911108] 
\draw    (159.15,689.55) .. controls (207.05,818) and (209.05,784) .. (260.5,714) ;
%Curve Lines [id:da7478198500849043] 
\draw    (159.15,788) .. controls (217.05,824) and (224.05,824) .. (260.5,760) ;

% Text Node
\draw (194.42,600) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {\scalebox{1}[1.1]{ReLU}\\ \scalebox{0.9}[1.1]{($n_j$)}};
% Text Node
\draw (263.24,730) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {\scalebox{0.9}[1.1]{$\link^{-1}$}\\
\scalebox{0.9}[1.1]{($d_j$)}};
% Text Node
\draw (129.07,729) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {\scalebox{1}[1.1]{Input}\\ \scalebox{0.9}[1.1]{($d_{j-1}$)} };

\end{tikzpicture}
\end{adjustbox}
\captionsetup{skip=5pt} % COULD COMMENT THIS MAYBE
\caption{Schematic representation of a shallow neural network with a trainable linear skip connection}
\label{fig:shallow_nn_skip}
\end{minipage}
\hfill
\begin{minipage}[t]{.3\linewidth}
\begin{adjustbox}{width=\linewidth,totalheight=1.5\linewidth}
\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,900); %set diagram left start at 0, and has height of 900

%Shape: Rectangle [id:dp9881686970179928] 
\draw   (124.05,689.55) -- (159.15,689.55) -- (159.15,788) -- (124.05,788) -- cycle ;
%Shape: Rectangle [id:dp021528437984906112] 
\draw   (189.96,489.09) -- (225.49,489.09) -- (225.49,732.64) -- (189.96,732.64) -- cycle ;
%Shape: Rectangle [id:dp9976069955613152] 
\draw   (260.5,714) -- (297.31,714) -- (297.31,760) -- (260.5,760) -- cycle ;
%Straight Lines [id:da7522636924221078] 
\draw    (159.15,689.55) -- (189.96,489.09) ;
%Straight Lines [id:da2407156240240318] 
\draw    (159.15,788) -- (189.96,732.64) ;
%Straight Lines [id:da5701929838169528] 
\draw    (225.49,489.09) -- (260.5,714) ;
%Straight Lines [id:da9714111484528329] 
\draw    (225.49,732.64) -- (260.5,760) ;
%Shape: Rectangle [id:dp6533761443859587] 
\draw   (188.05,776) -- (224.05,776) -- (224.05,822) -- (188.05,822) -- cycle ;
%Straight Lines [id:da426272438950303] 
\draw    (159.15,689.55) -- (188.05,776) ;
%Straight Lines [id:da6398129670593493] 
\draw    (159.15,788) -- (188.05,822) ;
%Straight Lines [id:da9259847557167127] 
\draw    (260.5,714) -- (224.05,776) ;
%Straight Lines [id:da09695599526203647] 
\draw    (260.5,760) -- (224.05,822) ;

% Text Node
\draw (194.42,600) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {\scalebox{1}[1.1]{ReLU}\\ \scalebox{0.9}[1.1]{($n_j$)}};
% Text Node
\draw (263.24,730) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {\scalebox{0.9}[1.1]{$\link^{-1}$}\\
\scalebox{0.9}[1.1]{($d_j$)}};
% Text Node
\draw (129.07,729) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {\scalebox{1}[1.1]{Input}\\ \scalebox{0.9}[1.1]{($d_{j-1}$)} };
% Text Node
\draw (191.19,790) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {\scalebox{1}[1.1]{Linear}\\
\scalebox{0.5}[0.75]{\fontsize{5}{6}\selectfont($\min(d_{j-1},d_j)$)}};

\end{tikzpicture}
\end{adjustbox}
%\captionsetup{skip=-5pt}
\caption{Schematic representation of a shallow neural network where many ($n_j$) hidden nodes have a ReLU activation and some ($\min(d_{j-1},d_j)$) hidden nodes have a linear (identity) activation function. Compared to \Cref{fig:shallow_nn_skip} the linear skip connection is factorized into two matrices.}
\label{fig:one_stack}
\end{minipage}

\end{figure}

==> Images/shematicThreeStacks.tex <==
\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,900); %set diagram left start at 0, and has height of 900

%Shape: Rectangle [id:dp008228614767346265] 
\draw   (73.05,208.55) -- (108.15,208.55) -- (108.15,307) -- (73.05,307) -- cycle ;
%Shape: Rectangle [id:dp5704329413062827] 
\draw   (138.96,72) -- (174.49,72) -- (174.49,277) -- (138.96,277) -- cycle ;
%Shape: Rectangle [id:dp4510734487688641] 
\draw   (209.5,259) -- (246.31,259) -- (246.31,305) -- (209.5,305) -- cycle ;
%Shape: Rectangle [id:dp02284685801621511] 
\draw   (280.42,72) -- (316.33,72) -- (316.33,277.45) -- (280.42,277.45) -- cycle ;
%Shape: Rectangle [id:dp93629233013766] 
\draw   (353.14,241.36) -- (389.05,241.36) -- (389.05,319.36) -- (353.14,319.36) -- cycle ;
%Straight Lines [id:da9888559282955649] 
\draw    (108.15,208.55) -- (138.96,72) ;
%Straight Lines [id:da09420527661413058] 
\draw    (108.15,307) -- (138.96,277) ;
%Straight Lines [id:da5672698781637233] 
\draw    (174.49,72) -- (209.5,259) ;
%Straight Lines [id:da9038073873782468] 
\draw    (246.31,259) -- (280.42,72) ;
%Straight Lines [id:da45145254545262614] 
\draw    (174.49,277) -- (209.5,305) ;
%Straight Lines [id:da5621136775375117] 
\draw    (246.31,305) -- (280.42,277.45) ;
%Straight Lines [id:da22909141129558508] 
\draw    (316.33,72) -- (353.14,241.36) ;
%Straight Lines [id:da7988859530231025] 
\draw    (316.33,277.45) -- (353.14,319.36) ;
%Shape: Rectangle [id:dp8976636437915166] 
\draw   (282.22,319.45) -- (317.23,319.45) -- (317.23,364) -- (282.22,364) -- cycle ;
%Straight Lines [id:da45244917183295086] 
\draw    (246.31,259) -- (282.22,319.45) ;
%Straight Lines [id:da3181466041377372] 
\draw    (246.31,305) -- (282.22,364) ;
%Straight Lines [id:da688828966240153] 
\draw    (317.23,319.45) -- (353.14,241.36) ;
%Straight Lines [id:da12231558965081613] 
\draw    (317.23,364) -- (353.14,319.36) ;
%Shape: Rectangle [id:dp016808137749252605] 
\draw   (136.78,319.45) -- (171.8,319.45) -- (171.8,364) -- (136.78,364) -- cycle ;
%Straight Lines [id:da014190844790572754] 
\draw    (108.15,208.55) -- (136.78,319.45) ;
%Straight Lines [id:da5888196906660979] 
\draw    (108.15,307) -- (136.78,364) ;
%Straight Lines [id:da9194765679939938] 
\draw    (171.8,319.45) -- (209.5,259) ;
%Straight Lines [id:da7177203643996719] 
\draw    (171.8,364) -- (209.5,305) ;
%Shape: Rectangle [id:dp5232562566788923] 
\draw   (423.42,73) -- (459.33,73) -- (459.33,278.45) -- (423.42,278.45) -- cycle ;
%Shape: Rectangle [id:dp26495238359049167] 
\draw   (496.14,261) -- (532.05,261) -- (532.05,306.45) -- (496.14,306.45) -- cycle ;
%Straight Lines [id:da26171249376784833] 
\draw    (389.05,241.36) -- (423.42,73) ;
%Straight Lines [id:da5159016275981532] 
\draw    (389.05,319.36) -- (423.42,278.45) ;
%Straight Lines [id:da12901460002976672] 
\draw    (459.33,73) -- (496.14,261) ;
%Straight Lines [id:da3198438831389272] 
\draw    (459.33,278.45) -- (496.14,306.45) ;
%Shape: Rectangle [id:dp47785938284248397] 
\draw   (425.22,320.45) -- (460.23,320.45) -- (460.23,365) -- (425.22,365) -- cycle ;
%Straight Lines [id:da19920004592020768] 
\draw    (389.05,241.36) -- (425.22,320.45) ;
%Straight Lines [id:da9523111262255173] 
\draw    (389.05,319.36) -- (425.22,365) ;
%Straight Lines [id:da44617005579536695] 
\draw    (460.23,320.45) -- (496.14,261) ;
%Straight Lines [id:da6733117316270143] 
\draw    (460.23,365) -- (496.14,306.45) ;

% Text Node
\draw (143.42,166) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {ReLU\\
($n_1$)};
% Text Node
\draw (284.98,166) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {ReLU\\
($n_2$)};
% Text Node
\draw (212.24,273) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {$\sigb$\\
($d_1$)};
% Text Node
\draw (354.83,273) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {$\sigb$\\
($d_2$)};
% Text Node
\draw (285.63,330) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {Linear\\
\scalebox{0.5}{\!\!($\min(d_1,d_2)$)}};
% Text Node
\draw (78.07,247) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {Input\\
($d_0$)};
% Text Node
\draw (140.19,330) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {Linear\\
\scalebox{0.5}{\!\!($\min(d_0,d_1)$)}};
% Text Node
\draw (427.98,167) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {ReLU\\
($n_3$)};
% Text Node
\draw (497.83,274) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {$\link^{-1}$\\
($d_3$)};
% Text Node
\draw (428.63,331) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {Linear\\
\scalebox{0.5}{\!\!($\min(d_2,d_3)$)}};

\end{tikzpicture}

==> Images/simplifiedThreeStacks.tex <==
\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,900); %set diagram left start at 0, and has height of 900

%Shape: Rectangle [id:dp008228614767346265] 
\draw   (73.05,208.55) -- (108.15,208.55) -- (108.15,307) -- (73.05,307) -- cycle ;
%Shape: Rectangle [id:dp5704329413062827] 
\draw   (138.96,72) -- (174.49,72) -- (174.49,277) -- (138.96,277) -- cycle ;
%Shape: Rectangle [id:dp4510734487688641] 
\draw   (209.5,259) -- (246.31,259) -- (246.31,305) -- (209.5,305) -- cycle ;
%Shape: Rectangle [id:dp02284685801621511] 
\draw   (280.42,72) -- (316.33,72) -- (316.33,277.45) -- (280.42,277.45) -- cycle ;
%Shape: Rectangle [id:dp93629233013766] 
\draw   (353.14,241.36) -- (389.05,241.36) -- (389.05,319.36) -- (353.14,319.36) -- cycle ;
%Straight Lines [id:da9888559282955649] 
\draw    (108.15,208.55) -- (138.96,72) ;
%Straight Lines [id:da09420527661413058] 
\draw    (108.15,307) -- (138.96,277) ;
%Straight Lines [id:da5672698781637233] 
\draw    (174.49,72) -- (209.5,259) ;
%Straight Lines [id:da9038073873782468] 
\draw    (246.31,259) -- (280.42,72) ;
%Straight Lines [id:da45145254545262614] 
\draw    (174.49,277) -- (209.5,305) ;
%Straight Lines [id:da5621136775375117] 
\draw    (246.31,305) -- (280.42,277.45) ;
%Straight Lines [id:da22909141129558508] 
\draw    (316.33,72) -- (353.14,241.36) ;
%Straight Lines [id:da7988859530231025] 
\draw    (316.33,277.45) -- (353.14,319.36) ;
%Shape: Rectangle [id:dp5232562566788923] 
\draw   (423.42,73) -- (459.33,73) -- (459.33,278.45) -- (423.42,278.45) -- cycle ;
%Shape: Rectangle [id:dp26495238359049167] 
\draw   (496.14,261) -- (532.05,261) -- (532.05,306.45) -- (496.14,306.45) -- cycle ;
%Straight Lines [id:da26171249376784833] 
\draw    (389.05,241.36) -- (423.42,73) ;
%Straight Lines [id:da5159016275981532] 
\draw    (389.05,319.36) -- (423.42,278.45) ;
%Straight Lines [id:da12901460002976672] 
\draw    (459.33,73) -- (496.14,261) ;
%Straight Lines [id:da3198438831389272] 
\draw    (459.33,278.45) -- (496.14,306.45) ;
%Curve Lines [id:da8450269290157659] 
\draw    (108.15,208.55) .. controls (156.05,341.36) and (135.05,339.36) .. (209.5,259) ;
%Curve Lines [id:da4914108654358684] 
\draw    (108.15,307) .. controls (129.05,372.36) and (181.05,348.36) .. (209.5,305) ;
%Curve Lines [id:da43414827659565325] 
\draw    (246.31,259) .. controls (277.05,361.36) and (335.05,341.36) .. (353.14,241.36) ;
%Curve Lines [id:da8456787563508839] 
\draw    (246.31,305) .. controls (266.05,375.36) and (323.05,356.36) .. (353.14,319.36) ;
%Curve Lines [id:da13137631557182772] 
\draw    (389.05,241.36) .. controls (437.94,373.18) and (459.05,313.36) .. (496.14,261) ;
%Curve Lines [id:da5862326697102673] 
\draw    (389.05,319.36) .. controls (419.05,361.36) and (487.05,360.36) .. (496.14,306.45) ;

% Text Node
\draw (143.42,166) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {ReLU\\
($n_1$)};
% Text Node
\draw (284.98,166) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {ReLU\\
($n_2$)};
% Text Node
\draw (212.24,273) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {$\sigb$\\
($d_1$)};
% Text Node
\draw (354.83,273) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {$\sigb$\\
($d_2$)};
% Text Node
\draw (79.07,247) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {Input\\
($d_0$)};
% Text Node
\draw (427.98,167) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {ReLU\\
($n_3$)};
% Text Node
\draw (497.83,274) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {$\link^{-1}$\\
($d_3$)};

\end{tikzpicture}
